Activity-Based Analysis of Open Source Software Contributors: Roles and Dynamics

Contributors to open source software (OSS) communities assume diverse roles to take different responsibilities. One major limitation of the current OSS tools and platforms is that they provide a uniform user interface regardless of the activities performed by the various types of contributors. This paper serves as a non-trivial first step towards resolving this challenge by demonstrating a methodology and establishing knowledge to understand how the contributors' roles and their dynamics, reflected in the activities contributors perform, are exhibited in OSS communities. Based on an analysis of user action data from 29 GitHub projects, we extracted six activities that distinguished four Active roles and five Supporting roles of OSS contributors, as well as patterns in role changes. Through the lens of the Activity Theory, these findings provided rich design guidelines for OSS tools to support diverse contributor roles.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> t_projectChangeClusters.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{0.8}
\centering
\small
\caption{Projects clustered based on trends in role composition change.}
\label{tab:ProjectsCluster}
\begin{tabular}{@{}cll@{}}
\toprule
\multicolumn{1}{l}{\textbf{Cluster}} & \multicolumn{1}{l}{\textbf{Project Name}} & \multicolumn{1}{l}{\textbf{Application/Domain}} \\

\midrule
\multirow{4}{*}{1} & adarkroom & Web game \\
 & picongpu & Science \\
 & primer & Design system \\
 & railsbridge/docs & Learn to code \\
 
\midrule
\multirow{7}{*}{2} & accessibility-developer-tools & Web accessibility \\
 & advocacy.mozilla.org & Web application \\
 & artsy.github.io & Blog \\
 & better\_errors & SE tool \\
 & guardian/frontend & Journalism \\
 & madison & Government \\
 & swipl-devel & Programming language \\
 
\midrule
\multirow{9}{*}{3} & cocos2d-html5 & JS game engine \\
 & hospitalrun-frontend & Healthcare \\
 & kubernetes & DevOps tool \\
 & mention-bot & OSS tool \\
 & neovim & Text editor \\
 & refined-github & Browser extention \\
 & superpowers-core & Game engine \\
 & TrueCraft & Game \\
 & urh & Wireless protocol tool\\

\bottomrule
\end{tabular}
\end{table}

==> t_roleClusterCount.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{0.8}
\centering
\small
\caption{Number of data points for each role cluster and number of projects each role appeared in}
\label{tab:ClusterCount}
\begin{tabular}{clcc}
\toprule
\textbf{Group} & \multicolumn{1}{c}{\textbf{Role Name}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Data\\Points\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Projects\end{tabular}} \\
\midrule
\multirow{4}{*}{Active} & All-Rounder & 1288 & 22\\
 & Coordinator & 159 & 4\\
 & Core Developer & 124 & 10\\
 & Intense Code Contributor & 10 & 3\\
\midrule
\multirow{5}{*}{Supporting} & Rare Contributor & 29943 & 29\\
 & Occasional Issue Reporter & 5284 & 29\\
 & Issue Fixer & 1294 & 23\\
 & Engaged Issue Reporter & 672 & 21\\
 & Progress Controller & 117 & 26\\
\bottomrule
\end{tabular}
\end{table}
